Ego-based Entropy Measures for Structural Representations on Graphs

Machine learning on graph-structured data has attracted high research interest due to the emergence of Graph Neural Networks (GNNs). Most of the proposed GNNs are based on the node homophily, i.e neighboring nodes share similar characteristics. However, in many complex networks, nodes that lie to distant parts of the graph share structurally equivalent characteristics and exhibit similar roles (e.g chemical properties of distant atoms in a molecule, type of social network users). A growing literature proposed representations that identify structurally equivalent nodes. However, most of the existing methods require high time and space complexity. In this paper, we propose VNEstruct, a simple approach, based on entropy measures of the neighborhood's topology, for generating low-dimensional structural representations, that is time-efficient and robust to graph perturbations. Empirically, we observe that VNEstruct exhibits robustness on structural role identification tasks. Moreover, VNEstruct can achieve state-of-the-art performance on graph classification, without incorporating the graph structure information in the optimization, in contrast to GNN competitors.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> VNEstruct_ICASSP (3)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> VNEstruct_ICASSP (3)/chapters/abstract.tex <==
Machine learning on graph-structured data has attracted high research interest due to the emergence of Graph Neural Networks (GNNs). Most of the proposed GNNs are based on the node homophily, i.e neighboring nodes share similar characteristics. However, in many complex networks, nodes that lie to distant parts of the graph share structurally equivalent characteristics and exhibit similar roles (e.g chemical properties of distant atoms in a molecule, type of social network users). A growing literature proposed representations that identify structurally equivalent nodes. However, most of the existing methods require high time and space complexity. In this paper, we propose \MN, a simple approach, based on entropy measures of the neighborhood's topology, for generating low-dimensional structural representations, that is time-efficient and robust to graph perturbations. Empirically, we observe that \MN exhibits robustness on structural role identification tasks. Moreover, \MN can achieve state-of-the-art performance on graph classification, without incorporating the graph structure information in the optimization, in contrast to GNN competitors.
% Moreover, on graph classification tasks, we suggest the utilization of the generated structural embeddings for the transformation of an attributed graph structure into a set of augmented node attributes.


% and state-of-the-art performance on graph classification tasks, while maintaining very high computational speed.

==> VNEstruct_ICASSP (3)/chapters/contribution.tex <==

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth,height=2.8cm]{figures/method.JPG}
    \caption{\MN extracts ego-networks for a series of defined radii and computes the VNE for every radius. On the left, the two parts of the network may have a large distance through the network. The 1-hop ego-networks are highlighted with the dark yellow, while the remaining nodes of the 2-hop ego-networks are highlighted with the light yellow. The nodes $u,v$ have structurally equivalent 1-hop neighborhoods $G_u^1$ and $G_v^1$, though their 2-hop neighborhoods $G_u^2$, $G_v^2$ do not.}
    \label{fig:method}
\end{figure*}


\section{Structural Representations based on Von Neumann Entropy}

Next, we present \MN for generating structural node representations, employing the Von Neumann entropy, a model-agnostic measure, that quantifies the structural complexity of a graph. The Von Neumann graph entropy (VNE) has been shown to have a linear correlation with other graph entropy measures~\cite{anand}. Graph entropy methods have been recently proved successful for computing graph similarity~\cite{lipan}.
% Our approach capitalizes on VNE to compute the similarity between neighborhoods of nodes and extract structural node representations. 

\subsection{Von Neumann Entropy on Graphs}

In quantum mechanics, the state of a quantum mechanical system is described by a \emph{density} matrix $\rho$, i.e., a positive semidefinite, hermitian matrix with unit trace~\cite{Braunstein2006}. The Von Neumann entropy of the quantum system is defined as: 
\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1.3pt}

\begin{equation}
    \label{eq::1}
    H(\rho) = -\Tr(\rho\log\rho) = -\sum_{i=1}^n \lambda_i\log\lambda_i,
\end{equation}
where $\Tr(\cdot)$ is the trace of a matrix, and $\lambda_i$'s are the eigenvalues of $\rho$.
Correspondingly, connecting it to graphs, given a graph $G=(V,E)$ and its Laplacian $L_G= D-A$, the VNE denoted by $H(G)$ , is defined as in Equation \ref{eq::1}, by replacing $\rho$ with $\rho(L_G) = \frac{L_G}{\text{Tr}(L_G)} = \frac{L_G}{2|E|}$~\cite{Braunstein2006}.
% Correspondingly, given a graph $G=(V,E)$ and its Laplacian $L_G= D-A$, the scaled matrix $\rho(L_G) = \frac{L_G}{\text{Tr}(L_G)} = \frac{L_G}{2|E|}$ is symmetric, positive semidefinite and with unit trace, suggesting an analogy with the density matrix~\cite{Braunstein2006}.
Note that $\lambda_i = \frac{1}{\text{Tr}(L_G)}v_i$ where $\lambda_i, v_i$ are the $i$-th eigenvalue of $\rho(L_G)$ and $L_G$, respectively. Therefore, $0 \leq \lambda_i \leq 1$ holds for all $i \in \{ 0,1,\ldots,n \}$~\cite{Passerini2009QuantifyingCI}.
This indicates that \Eqref{eq::1} is equivalent to the Shannon entropy of the probability distribution $\{\lambda_i\}_{i=1}^n$.
Hence, $H(G)$ serves as a skewness metric of the eigenvalue distribution and it has been shown that it provides information on the structural complexity of a graph~\cite{Passerini2009QuantifyingCI}.

\textbf{Efficient approximation scheme.}
The computation of VNE requires the eigenvalue decomposition of the density matrix which can be done in $\mathcal{O}(n^3)$ time. Recent works~\cite{fast_incr, choi2018fast} have proposed an efficient approximation of $H(G)$. Starting from \Eqref{eq::1} and following~\cite{minello}, we obtain:
\begin{equation}\label{eq::3}
    H(G) \approx \text{Tr}\big(\rho(L_G)(I_n - \rho(L_G))\big) = Q,
\end{equation}
where $I_n$ is the $n \times n$ identity matrix, and
\setlength\abovedisplayskip{1pt}
\setlength\belowdisplayskip{1pt}

\begin{equation}\label{eq::4}
        Q = \frac{\text{Tr}(L_G)}{2m} - \frac{\text{Tr}(L_G^2)}{4m^2}
        = 1 - \frac{1}{2m} - \frac{1}{4m^2}\sum_{i=1}^n d_i^2\,,
\end{equation}
where $m=|E|$ and $d_i$ is the ith-node degree. Finally, as~\cite{fast_incr} suggests, we obtain a tighter approximation of $H(G)$:
\setlength\abovedisplayskip{1.3pt}
\setlength\belowdisplayskip{1.3pt}

\begin{equation}\label{eq::5}
 \hat{H} = -Q\ln\lambda_{\max}\,,
\end{equation}

where $\lambda_{\max}$ is the largest eigenvalue of $\rho(L(G))$.
It can be shown that for any graph $G$, we have $H(G) \geq \hat{H}(G)$ where the equality holds if and only if $\lambda_{\max} = 1$~\cite{choi2018fast}.

\begin{table*}[t]
\centering
% \scriptsize
\def\arraystretch{1.1}
% \begin{sc}
\resizebox{\textwidth}{!}{
\begin{tabular}{|lc|l||ccc|cc|} \hline
Configuration & Shapes & Algorithm & Homogeneity & Completeness & Silhouette & Accuracy & F$1$-score \\ \hline
\multirow{7}{*}{Basic / Basic Perturbed} & \multirow{7}{*}{\includegraphics[width=.2\textwidth]{figures/shapes2.pdf}} & DeepWalk & 0.178 / 0.172 & 0.115 / 0.124 & 0.163 / 0/171 & 0.442 / 0.488 & 0.295 / 0.327 \\
& & RolX& 0.983 / 0.764 & 0.976 / 0.458 & 0.846 / 0.429 & \textbf{1.000} / 0.928 & \textbf{1.000} / \textbf{0.886} \\
& & struc2vec& 0.803 / 0.625 & 0.595 / 0.543 & 0.402 / 0.429 & 0.784 / 0.703 & 0.708 / 0.632 \\
& & GraphWave& 0.868 / 0.714 & 0.797 / 0.326 & 0.730 / 0.287 & 0.995 / 0.906 & 0.993 / 0.861 \\
& & VNEstruct& \textbf{0.986} / \textbf{0.882} & \textbf{0.983} / \textbf{0.701} & \textbf{0.891} / \textbf{0.478} & 0.920 / \textbf{0.940} & 0.901 / 0.881 \\ \hline

\multirow{7}{*}{Varied / Varied Perturbed} &
\multirow{7}{*}{\includegraphics[width=.2\textwidth]{figures/shapes5.pdf}} & DeepWalk& 0.327 / 0.300 & 0.220 / 0.231 & 0.216 / 0.221 & 0.329 / 0.313 & 0.139 / 0.128 \\
& & RolX& \textbf{0.984} / 0.682  & 0.939 / 0.239 & 0.748 / 0.062 & \textbf{0.998} / 0.856 & 0.996 / 0.768 \\
& & struc2vec& 0.805 / 0.643 & 0.626 / 0.524 & 0.422 / \textbf{0.433} & 0.738 / 0.573 & 0.592 / 0.412 \\
& & GraphWave& 0.941 / 0.670 & 0.843 / 0.198 & \textbf{0.756} / 0.005 & 0.982 / 0.793 & \textbf{0.965} / 0.682 \\ 
& & VNEstruct& 0.950 / \textbf{0.722}  & \textbf{0.945} / \textbf{0.678} & 0.730 / 0.399 & 0.988 / \textbf{0.899} & 0.95 \textbf{0.878} \\ \hline 
\hline 
\end{tabular}
}
\caption{Performance of the baselines and the VNEstruct method for learning structural embeddings averaged over $20$ synthetically generated graphs. Dashed lines denote perturbed graphs.}
% \end{sc}
\label{tab:shapes}
\end{table*}

\subsection{The \MN Algorithm}
Based on the VNE and its approximation, we introduce our proposed approach to construct structural representations. The \MN algorithm extracts ego-networks of increasing radius and computes their VNE.
Then, the representation of a node comprises of the Von Neumann entropies that emerged from the node's ego-networks.
Therefore, the set of entropies of the ego-networks of a node serves as a ``signature'' of the structural identity of its neighborhood.

Let $R$ be the maximum considered radius. For each $r \in \{1,..,R\}$ and each node $v \in V$, the algorithm extracts the $r$-hop neighborhood  $G_v^r = (V',E')$, where $V' = \{u \in V | d(u,v) \leq r\}$ and $E' = \{(u,v) | u, v \in V', (u,v) \in E \}$.
Next, $H(G_v^r)$ of the $r$-hop neighborhood of $v$ is computed using \Eqref{eq::5}.
Finally, the $R$ entropies are arranged into a single vector $h_v \in \mathbb{R}^R$. As shown in Figure~\ref{fig:method}, \MN identifies structural equivalences of nodes that are distant to each other. Specifically, nodes $u$ and $v$ share structurally identical $1$-hop neighborhoods.
Therefore, the entropies of their $1$-hop neighborhoods are equal to each other.
% However, this is not the case for the entropies of their $2$-hop neighborhoods since the two subgraphs are very dissimilar from each other.
%Note that in this work, we focus on undirected graphs without edge weights.  However, our approach easily extends in the case of weighted and directed graphs.

\makeatletter
\newcommand{\removelatexerror}{\let\@latex@error\@gobble}
\makeatother

% \bigskip
% \vspace{1mm}
% \begingroup
% \removelatexerror% Nullify \@latex@error
% \begin{algorithm}[H]
% \SetAlgoLined
% \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% \SetKwFor{ForEach}{foreach}{do}{endfor}
 
% \Input{graph $G=(V,E)$, radius $R$}
% \Output{An embedding matrix $H \in \mathbb{R}^{n\times R}$ }
%  \ForEach{$v \in V$}{
%     \ForEach{$r \in \{1,\ldots,R\}$}{
%     Extract ego-graph Laplacian $L_{G_v^r}$\\
%     Derive density matrix $\rho(L_{G_v^r}) = \frac{L_{G_v^r}}{\text{Tr}(L_{G_v^r})}$\\
%     $ \lambda_{\max} \leftarrow \text{Power-Iteration}(\rho(L_{G_v^r}))$\\
%     $Q \leftarrow 1 - \frac{1}{2m} - \frac{1}{4m^2}\sum_{i=1}^{|V'|} d_i^2$
    
%     $h(v,r) \leftarrow -Q \ln\lambda_{\max}$ 
%     }
%     $H_v \leftarrow$ CONCAT$(h(v,1),...,h(v,R))$
%  }
%  \caption{\MN algorithm}
%  \label{algo:vne}
% \end{algorithm}
% \endgroup

\textbf{Computational Complexity.}
The algorithm consists of: ($1$) the extraction of the ego-networks and ($2$) the computation of VNEs per subgraph.
The first step is linear in the number of edges of the node's neighborhood.
In the worst case, the complexity is $\mathcal{O}(nm)$, but for sparse graphs the complexity is constant in practice.
For the second step, following the approximation scheme in subsection 2.1, 
$\lambda_{max}$ is computed through the power iteration method~\cite{power_iteration}, which requires $\mathcal{O}(n+m)$ operations, as the Laplacian matrix has $n+m$ nonzero entries. 
% we do not perform the eigenvalue decomposition of the \emph{density} matrix (requires $\mathcal{O}(n^3)$ time), but we make use of \Eqref{eq::5}.
% This requires finding the largest eigenvalue $\lambda_{max}$ and computing simple degree statistics for each $r$-hop neighborhood.  
% We use the power iteration method~\cite{power_iteration} to compute $\lambda_{max}$, which requires $\mathcal{O}(n+m)$ operations, as the Laplacian matrix has $n+m$ nonzero entries.
Hence, the whole method exhibits linear complexity $\mathcal{O}(n+m)$, while for very sparse graphs, it becomes $\mathcal{O}(n)$.  

\textbf{Robustness over "small" perturbations.} We will next show that utilizing the VNE, we can acquire robust structural representations over possible perturbations on the graph structure. Clearly, if two graphs are isomorphic to each other, then their entropies will be equal to each other. It is important, though, for structurally similar graphs to have similar entropies, too. So, let $\rho, \rho' \in \mathbb{R}^{n \times n}$ be the density matrices of two graph laplacians $L_G,L_{G'}$, as described above.
Let also $\rho = P \rho' P^\top + \epsilon$ where $P$ is an $n \times n$ permutation matrix equal to $\argmin_{P} || \rho - P \rho' P^\top ||_F$ and $\epsilon$ is an $n \times n$ symmetric matrix.
If $G,G'$ are nearly-isomorphic, then the Frobenius norm of $\epsilon$ is small. By applying the Fannes-Audenaert inequality~\cite{Audenaert_2007}, we have that:
\begin{equation*}
 |H(\tilde{\rho}) - H(\rho)| \leq \frac{1}{2}T \ln(n-1) + S(T),   
\end{equation*} where $T = ||\tilde{\rho}-\rho||_1$ is the trace distance between $\rho,\tilde{\rho}$ and $S(T) = -T\log T- (1-T)\log(1-T)$.
However, $||\tilde{\rho}-\rho||_1 = \sum_i|\lambda_i^{\tilde{\rho}-\rho}| \leq n||\tilde{\rho} - \rho ||_{op}$, where $|| \cdot ||_{op}$ is the operator norm.
Therefore, $|H(\tilde{\rho})- H(\rho)| \leq \frac{n}{2}ln(n-1)||\epsilon||_{op} + S(T)$, leading thus to a size-dependent upper bound of the difference between the entropies of structurally similar graphs. 





\subsection{Graph-level Representations}
Next, we propose how the structural representations generated by \MN can be combined with node attributes to perform graph classifications tasks.
The majority of the state-of-the-art methods learn node representations using message-passing schemes~\cite{hamilton, xu2018powerful}, where each node updates its representation according to its neighbors' representations, utilizing the graph structure information.

% Clearly, each time the nodes update their representations, the structure of the graph is taken into account.
In this work, we do not use any message-passing scheme and we ignore the graph structure.
Instead, we augment the node attribute vectors of a graph with the structural representations generated by \MN. % employ the \MN and we embed the nodes into a low-dimensional space.
% These embeddings are then combined with the node attributes (if any).
% This forms the pre-processing, feature extraction step.
Thus, information about the graph structure is implictly incorporated into the augmented node attributes. Given a matrix of node attributes $X \in \mathbb{R}^{n\times d}$, the approach performs the following steps:

\begin{itemize}
    \itemsep0em 
    \item Computation of $H_v \in \mathbb{R}^{n\times R}$.
    \item Concatenation of node attribute vectors with structural node representations: $X' = [X || H] \in \mathbb{R}^{n\times (d+R)}$.
    \item Aggregation of node vectors $X'$ into:\\ $H_G = \psi( \sum_{v \in V_G} \phi(X'_v)) $, where $\phi$ and $\psi$ are MLPs.
\end{itemize}

This approach is on par with recent studies that propose to augment the node attributes with structural characteristics to avoid performing message-passing steps~\cite{DBLP:journals/corr/abs-1905-04579}. 
In comparison to a GNN, this procedure reduces the computational complexity of the training procedure since each graph is represented as a set of node representations.









==> VNEstruct_ICASSP (3)/chapters/experiments.tex <==


\section{Experiments}
Next, we empirically show the robustness that \MN exhibits to graph perturbations in subsection 3.1 and we evaluate its graph classification performance in subsection 3.2.
% For the structural role identification task we use both synthetic and real-world graphs, while for the graph classification task we use 5 well-studied real-world datasets.

\subsection{Structural Role Identification}
% We first experiment with some synthetic datasets and then we compare the performance of \MN and baselines on a real-world dataset.

% \subsubsection{Highly-symmetrical synthetic networks}
In order to evaluate the robustness of the structural representations generated by our method, we measure its performance on perturbed synthetic datasets, which were introduced in~\cite{donat, DBLP:journals/corr/FigueiredoRS17}.
We perform both classification and clustering tasks with the same experimental setup as in~\cite{donat}.\\
\textbf{Dataset setup.} The generated synthetic datasets are identical to those used in~\cite{donat}. They consist of basic symmetrical shapes, as shown in Table~\ref{tab:shapes}, that are regularly placed along a cycle of length $30$. The \textit{basic} setups use 10 instances of only one of the shapes of Table~\ref{tab:shapes}, while the \textit{varied} setups use 10 instances of each shape, randomly placed along the cycle. 
The perturbed instances are formed by randomly rewiring edges.
The colors in the shapes indicate the different classes.\\
\textbf{Evaluation.} For the classification task, we measure the \textit{accuracy} and the \textit{F1-score}. 
For the clustering task, we report the $3$ evaluation metrics, that were also calculated in~\cite{donat}: the \textit{Homogeneity} evaluates the conditional entropy of the structural roles in the produced clustering result, the  \textit{Completeness} evaluates how many nodes with equivalent structural roles are assigned to the same cluster and the \textit{Silhouette} measures the intra-cluster distance vs. the inter-cluster distance. 


% \begin{table*}[ht]
% \centering
% % \scriptsize
% \def\arraystretch{1.1}
% % \begin{sc}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|lc|l||ccc|cc|} \hline
% Configuration & Shapes & Algorithm & Homogeneity & Completeness & Silhouette & Accuracy & F$1$-score \\ \hline
% \multirow{7}{*}{Basic / Basic Perturbed} & \multirow{7}{*}{\includegraphics[width=.2\textwidth]{figures/shapes2.pdf}} & DeepWalk & 0.178 / 0.172 & 0.115 / 0.124 & 0.163 / 0/171 & 0.442 / 0.488 & 0.295 / 0.327 \\
% & & RolX& \textbf{0.983} / 0.764 & \textbf{0.976} / 0.458 & 0.846 / 0.429 & \textbf{1.000} / 0.928 & \textbf{1.000} / \textbf{0.886} \\
% & & struc2vec& 0.803 / 0.625 & 0.595 / 0.543 & 0.402 / 0.429 & 0.784 / 0.703 & 0.708 / 0.632 \\
% & & GraphWave& 0.868 / 0.714 & 0.797 / 0.326 & 0.730 / 0.287 & 0.995 / 0.906 & 0.993 / 0.861 \\
% & & VNEstruct& 0.966 / \textbf{0.882} & 0.963 / \textbf{0.701} & \textbf{0.891} / \textbf{0.478} & 0.920 / \textbf{0.940} & 0.901 / 0.881 \\ \hline

% \multirow{7}{*}{Varied / Varied Perturbed} &
% \multirow{7}{*}{\includegraphics[width=.2\textwidth]{figures/shapes5.pdf}} & DeepWalk& 0.327 / 0.300 & 0.220 / 0.231 & 0.216 / 0.221 & 0.329 / 0.313 & 0.139 / 0.128 \\
% & & RolX& \textbf{0.984} / 0.682  & \textbf{0.939} / 0.239 & 0.748 / 0.062 & \textbf{0.998} / 0.856 & 0.996 / 0.768 \\
% & & struc2vec& 0.805 / 0.643 & 0.626 / 0.524 & 0.422 / \textbf{0.433} & 0.738 / 0.573 & 0.592 / 0.412 \\
% & & GraphWave& 0.941 / 0.670 & 0.843 / 0.198 & \textbf{0.756} / 0.005 & 0.982 / 0.793 & \textbf{0.965} / 0.682 \\ 
% & & VNEstruct& 0.950 / \textbf{0.722}  & 0.892 / \textbf{0.678} & 0.730 / 0.399 & 0.988 / \textbf{0.899} & 0.95 \textbf{0.878} \\ \hline 
% \hline 
% \end{tabular}
% }
% \caption{Performance of the baselines and the \textit{VNEstruct} method for learning structural embeddings averaged over $20$ synthetically generated graphs. Dashed lines denote perturbed graphs.}
% % \end{sc}
% \label{tab:shapes}
% \end{table*}


In Table~\ref{tab:shapes}, VNEstruct outperforms the competitors on the perturbed instances of the synthetic graphs. On the basic and varied configurations, \MN outperforms the competitors in the node clustering evaluation and achieves comparable performance with RolX in node classification. On the perturbed configurations, \MN exhibits stronger performance than its competitors. The results in Table~\ref{tab:shapes} suggest a comparison of VNEstruct, RolX, and GraphWave in noisy scenarios. This comparison is provided in \Figref{fig:performances}, where we report the performance with respect to the number of rewired edges (from $0$ to $20$). We see that \MN is more robust than GraphWave and Rolx in the presence of noise.

% \subsubsection{Role identification on Email-dataset}
% We next evaluate the performance of VNEstruct algorithm and of its competitors on a real-world dataset, the Enron Email dataset~\cite{enron}.
% This is an email network, where nodes are company employees with one of seven different positions (e.g. CEO, Manager, Employee etc.) and the edges indicate the email communication. It contains 143 nodes and 2,583 edges. We consider that nodes with structurally similar positions in the graph share similar roles. Following the same experimental protocol as in~\cite{donat}, we generate  structural embeddings.
% Regarding the \MN, we hyperparameterized over the radius $r \in \{1,2,3\}$, since the graph diameter is 4.
% Table~\ref{tab::enron} shows that \MN  with  radius $R=3$ and a low embedding dimensionality ($d\leq 3$) achieves competitive results with strong baselines, which produce embeddings with higher dimensionality ($d>10$).

% \begin{table}[htp]
% % \scriptsize
% \centering
% \begin{tabular}{|l|cccc|}
% \hline
%  Method    & C  & H    & S & Dimension    \\ \hline
%  RolX      & 0.028          & 0.090          & 0.425 & 16 - 32          \\ 
%  struc2vec & 0.018          & 0.003          & 0.435 & 64 - 128         \\ 
%  GraphWave & \textbf{0.067} & \textbf{0.115} & 0.577 & 50 - 100         \\ 
%  \MN & 0.049          & 0.107          & \textbf{0.591} & 1 - 3 \\ \hline
% \end{tabular}

% \caption{Clustering evaluation for Enron Email. C, H, S stand for Completeness, Homogeneity and Silhouette.}
% \label{tab::enron}
% \end{table}
% \vspace{-0.7cm}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.3\textwidth]{figures/performances_together2.jpeg}
    \caption{Classification and clustering performance of \MN and the baselines with respect to noise.}
    \label{fig:performances}
\end{figure}




\subsection{Graph Classification}
Next, we evaluate \MN and the baselines in the task of graph classification. We compare our proposed algorithm against well-established message-passing algorithms for learning graph representations.
Note that in contrast to most of the baselines, we pre-compute the entropy-based structural representations, and then we represent each graph as a set of vectors that encode structural characteristics. We used 4 common graph classification datasets (3 from bioinformatics: MUTAG, PROTEINS, PTC-MR and 1 from social-networks: IMDB-BINARY~\cite{xu2018powerful}). 

\textbf{Baselines.} The goal of the comparison is to show that by decomposing the graph structure and the attribute space, we can achieve comparable results to the state-of-the-art algorithms. Thus, we use as baselines graph neural network variants and specifically: DGCNN~\cite{Zhang2018AnED}, Capsule GNN~\cite{Xinyi2019CapsuleGN}, GIN~\cite{xu2018powerful}, GCN~\cite{Kipf:2016tc}, GAT~\cite{gat}. Moreover, GFN~\cite{DBLP:journals/corr/abs-1905-04579} augments the attributes with structural features and ignores the graph structure during the learning procedure. 


\textbf{Model setup.}
For the baselines, we followed the same experimental setup, as described in~\cite{DBLP:journals/corr/abs-1905-04579} and, thus, we report the achieved accuracies. For GAT, we used a summation operator as an aggregator of the node vectors into a graph-level representation. Regarding the \MN, we performed 10-fold cross-validation with Adam optimizer and a 0.3 learning rate decay every 50 epochs. In all experiments, we set the number of epochs to 300. We choose the radius of the ego-networks from $r \in \{1,2,3,4\}$ and the number of hidden layers of the MLPs from $d \in \{8,16,32\}$.

% \paragraph{Performance and efficiency results.}

Table~\ref{tab::graphclass} illustrates the average classification accuracies of the proposed approach and the baselines on the $5$ graph classification datasets.
Interestingly, the proposed approach achieves accuracies comparable to those of the state-of-the-art message-passing models. \MN outperformed all the baselines on $3$ out of $4$ datasets, while achieved the second-best accuracy on the remaining dataset (i.e., PROTEINS).


\begin{figure}[h!]
    \centering
    \includegraphics[width=1.\columnwidth, height=4.2cm]{figures/speed2.jpeg}
    \caption{Training time per epoch (in sec) of VNEstruct and competitors for the graph classification tasks. }
    \label{fig:speed}
\end{figure}

\begin{table}[t]
% \setlength{\tabcolsep}{1pt}
% \scriptsize
\centering
\resizebox{0.47\textwidth}{!}{

\begin{tabular}{|c|cccc|}
\hline
  Method    & MUTAG   & IMDB-BINARY    & PTC-MR & PROTEINS     \\ \hline
  DGCNN      &  85.83 $\pm$ 1.66 & 70.03 $\pm$ 0.86 & 58.62$\pm$2.34 & 75.54 $\pm$ 0.94 \\ 
 
  CapsGNN      & 86.67 $\pm$ 6.88          & 73.10 $\pm$ 4.83         & - & 76.28 $\pm$ 3.63 \\ 
  GAT & 88.90 $\pm$ 3.21 & 75.39 $\pm$ 1.30 &  63.87 $\pm$ 5.31 &  76.1 $\pm$ 2.89 \\
  GIN & 89.40 $\pm$ 5.60 & 75.10 $\pm $ 5.10          & 64.6 $\pm$ 7.03 & 76.20 $\pm$ 2.60  \\ 
   GCN & 87.20 $\pm$ 5.11  & 73.30 $\pm$ 5.29 & 64.20 $\pm$ 4.30  & 75.65 $\pm$ 3.24 \\ 
\hline
  GFN & 90.84 $\pm$ 7.22 & 73.00 $\pm$ 4.29 & - &  \textbf{77.44 $\pm$ 3.77}\\ 
  \MN & \textbf{91.08 $\pm$ 5.65 }         & \textbf{75.40 $\pm$ 3.33}          & \textbf{65.39 $\pm$ 8.57}  & 77.41 $\pm$ 3.47  \\ 
  \hline
\end{tabular}
}
\caption{Average classification accuracy ($\pm$ standard deviation) of the baselines and the proposed \MN.}

\label{tab::graphclass}
\end{table}

Figure~\ref{fig:speed} illustrates the average training time per epoch of \MN and the baselines that apply message-passing schemes.
The proposed approach is generally more efficient than the baselines.
Specifically, it is $0.31$ times faster than GIN and $0.60$ times faster than GCN on average.
This improvement in efficiency is mainly because the graph structural features are computed in a preprocessing step and are then concatenated with the node attributes. However, the computational cost of the preprocessing step is negligible, as it is performed only once in the experimental setup. Furthermore, we should mention that due to the low dimensionality of the generated embeddings ($d \leq 4$), our method does not have any significant requirements in terms of memory.




\section{Conclusion}

In this paper, we proposed \MN to generate structural node representations, based on the entropies of ego-networks. We showed empirically the robustness of \MN under the presence of noise in the graph. We, also, proposed an approach for performing graph classification, that combines the representations of \MN with the nodes' attributes, avoiding the computational cost of message passing schemes. The proposed approach exhibited a strong performance in real-world datasets, maintaining high efficiency. 

==> VNEstruct_ICASSP (3)/chapters/introduction.tex <==
\section{Introduction}

The amount of data that can be represented as graphs has increased significantly in recent years. Graph representations are ubiquitous in several fields such as in biology, chemistry~\cite{pmlr-v70-gilmer17a}, and social networks~\cite{hamilton}.
Many applications require performing machine learning tasks on graph-structured data, such as graph classification~\cite{xu2018powerful}, semi-supervised node classification~\cite{Kipf:2016tc} and link prediction~\cite{kipf2016variational}.% For instance, in chemistry, graph regression can successfully replace expensive quantum mechanical simulation approaches in predicting molecular properties ~\cite{pmlr-v70-gilmer17a}. 

The past few years have witnessed great activity in the field of learning on graphs. Graph Neural Networks (GNNs) have emerged as a successful approach on learning node-level and graph-level representations. %have achieved great success in tackling both node and graph-related problems~\cite{Kipf:2016tc, xu2018powerful, hamilton}. 
Recently, the interest on this field has focused on the expressiveness of GNNs~\cite{xu2018powerful,clip} and how these models can be deep enough to extract long-range information from distant nodes in the graph~\cite{deeperinsight,pairnorm,khop}. So far, most of the models are designed so that they preserve the proximity between nodes, i.e., nodes that are close to each other in the graph obtain similar representations~\cite{hamilton, perozzi2014deepwalk}. However, some tasks require assigning similar representations to nodes that can be distant in the graph, but structurally equivalent. For example, in chemistry, properties of a molecule often depend on the interaction of the atoms at its oposite sides and their neighborhood topology~\cite{deepatoms}. 
These tasks require \emph{structural representations}, i.e. embeddings that can identify structural properties of a node's neighborhood. There is a growing literature that adresses this problem through different approaches. RolX ~\cite{rolx} extracts features for each node and performs non-negative matrix factorization to automatically discover node roles. Struc2vec~\cite{DBLP:journals/corr/FigueiredoRS17},
performs random walks on a constructed multi-layer graph to learn structural representations. GraphWave~\cite{donat} and DRNE~\cite{drne} employ diffusion wavelets and LSTM aggregation operators, respectively, to generate structural node embeddings.
However, most of these approaches suffer from high time or space complexity. % One main drawback of this method is that it suffers from high space complexity.  aggregates neighborhood information using an LSTM operator. This method implies an ordering of each node's neighborhood, hence not satisfying the permutation invariance criteria.  
% Regarding the utilization of structural characteristics in order to decompose the graph structure and the attribute space of the graph nodes, a recent work~\cite{DBLP:journals/corr/abs-1905-04579} proposes the augmentation of the node attribute vectors with features that encode the graph structure. 

In this paper, we propose a novel and simple structural node representation algorithm, \MN, that capitalizes on information-theoretic tools. The algorithm employs the Von Neumann entropy to construct node representations related to the structural identity of the neighborhood of each node. These representations capture the structural symmetries of the neighborhoods of increasing radius of each node. We show empirically the ability of \MN to identify structural roles and its robustness to graph perturbations through a node classification and node clustering study on highly symmetrical synthetic graphs.  
Moreover, we introduce a method of combining the generated representations by \MN with the node attributes of a graph, in order to avoid the incorporation of the graph topology in the optimization, contrary to the workflow of a GNN. Evaluated on real-world graph classification tasks, \MN achieves state-of-the-art performance, while maintaining a high efficiency compared to standard GNN models.   


==> VNEstruct_ICASSP (3)/definitions.tex <==
% My package imports and snippets
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{hyperref}
\usepackage{url}
\usepackage{graphicx,wrapfig}  
\usepackage{nccmath}
% \usepackage[dvipsnames]{xcolor}
\usepackage{amsmath}
\newcommand{\todo}[1]{\textcolor{red}{#1}}
\newcommand{\kevin}[1]{\textcolor{green}{(kevin: #1)}}
\newcommand{\aladin}[1]{\textcolor{ForestGreen}{(aladin: #1)}}
% For references
\newcommand{\Sec}[1]{Section~\ref{sec:#1}}
\newcommand{\Eq}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\Alg}[1]{Alg.~(\ref{alg:#1})}
\newcommand{\Tab}[1]{Tab.\,\ref{#1}}
\newcommand{\Fig}[1]{Figure~\ref{fig:#1}}
\newcommand{\Def}[1]{Definition~\ref{def:#1}}
\newcommand{\Theorem}[1]{Theorem~\ref{th:#1}}
\newcommand{\Proposition}[1]{Proposition~\ref{prop:#1}}
\newcommand{\Corollary}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Lemma}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Appendix}[1]{Appendix~\ref{appendix:#1}}
\newcommand{\Supplementary}[1]{Supplementary~\ref{appendix:#1}}
\newcommand{\Table}[1]{Table~\ref{tab:#1}}


\newcommand{\MethodName}{Von Neumann Structural Embedding\xspace}
\newcommand{\MN}{VNEstruct\xspace}


% In your preamble

\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

==> VNEstruct_ICASSP (3)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\tr}{tr}

